Identifying Cache-Based Side Channels through Secret-Augmented Abstract Interpretation

Cache-based side channels enable a dedicated attacker to reveal program secrets by measuring the cache access patterns. Practical attacks have been shown against real-world crypto algorithm implementations such as RSA, AES, and ElGamal. By far, identifying information leaks due to cache-based side channels, either in a static or dynamic manner, remains a challenge: the existing approaches fail to offer high precision, full coverage, and good scalability simultaneously, thus impeding their practical use in real-world scenarios. In this paper, we propose a novel static analysis method on binaries to detect cache-based side channels. We use abstract interpretation to reason on program states with respect to abstract values at each program point. To make such abstract interpretation scalable to real-world cryptosystems while offering high precision and full coverage, we propose a novel abstract domain called the Secret-Augmented Symbolic domain (SAS). SAS tracks program secrets and dependencies on them for precision, while it tracks only coarse-grained public information for scalability. We have implemented the proposed technique into a practical tool named CacheS and evaluated it on the implementations of widely-used cryptographic algorithms in real-world crypto libraries, including Libgcrypt, OpenSSL, and mbedTLS. CacheS successfully confirmed a total of 154 information leaks reported by previous research and 54 leaks that were previously unknown. We have reported our findings to the developers. And they confirmed that many of those unknown information leaks do lead to potential side channels.

==> design-check.tex <==
\textbf{Checking with the Constraint Solver}

upon the fix point of analyzing each function, we check formulas of each memory
load and store instruction. When a secret-dependent abstract value $a \in
\mathbf{AV}_{s}$ is identified, its corresponding memory access instruction is
considered to be ``secret-dependent.'' \caches\ then translates each abstract
value $a \in \mathbf{AV}_{s}$ into a SMT formula $f$ for constraint checking.

At this step \caches\ adopts the cache model proposed by existing work to check
each secret-dependent memory access~\cite{wang2017cached}. Given $f$
translated from $a \in \mathbf{AV}_{s}$ 
that represents a memory address (see \S~\ref{subsec:design-smt}), \caches checks potential cache line
access variants by solving the satisfiability of the following predicate:

\begin{equation} \label{eq:formula}
  f \rs L \neq f[sv_{i}\mapsto sv'_i] \rs L
\end{equation}
\noindent where $sv_{i}$ is a bit vector with respect to one 
secret symbol $s_{i}$, and $sv_{i}'$ is another fresh bit vector corresponding to each $sv_{i}$.

As discussed in \S~\ref{sec:background}, assuming the cache has the line size
of $2^L$ bytes, for a memory address of $N$ bits, the upper $N-L$ bits map a
memory access to its corresponding cache line access. In other words, the upper
$N-L$ bits decide which cache line the upcoming memory access would visit.
Therefore, for an SMT formula $f$ derived from $a \in \mathbf{AV}_s$, we right shift $f$
by $L$ bits, and the result $f\rs L$ indicates the cache line being
accessed. Furthermore, by replacing each $sv_{i}$ with another 
bit vector $sv'_{i}$, we obtain $f[sv_{i}\mapsto sv'_{i}] \rs
L$.

We then construct the aforementioned constraint (\ref{eq:formula}), which checks whether
different secrets ($s_{i}$ and $s_{i}'$) can lead to
the access of different cache lines at this memory access. Recall the threat model shown in \F~\ref{fig:threat-model}, 
the existence of at
least one satisfiable solution reveals the side channels at this point.
From an attacker's perspective, by (indirectly) observing the access of different cache lines, a
certain amount of secrets could be leaked to adversaries. As a standard
setting, the cache line size is assumed to be 64 ($2^6$) in this work; therefore, we
set $L$ as 6.

In addition, since $\top$ implies that a variable has some residual secrets
along with possibly public information, memory accesses are conservatively
marked as vulnerable whenever their corresponding addressing formulas are
$\top$.

